DSC-PoseNet: Learning 6DoF Object Pose Estimation via Dual-scale Consistency

Compared to 2D object bounding-box labeling, it is very difficult for humans to annotate 3D object poses, especially when depth images of scenes are unavailable. This paper investigates whether we can estimate the object poses effectively when only RGB images and 2D object annotations are given. To this end, we present a two-step pose estimation framework to attain 6DoF object poses from 2D object bounding-boxes. In the first step, the framework learns to segment objects from real and synthetic data in a weakly-supervised fashion, and the segmentation masks will act as a prior for pose estimation. In the second step, we design a dual-scale pose estimation network, namely DSC-PoseNet, to predict object poses by employing a differential renderer. To be specific, our DSC-PoseNet firstly predicts object poses in the original image scale by comparing the segmentation masks and the rendered visible object masks. Then, we resize object regions to a fixed scale to estimate poses once again. In this fashion, we eliminate large scale variations and focus on rotation estimation, thus facilitating pose estimation. Moreover, we exploit the initial pose estimation to generate pseudo ground-truth to train our DSC-PoseNet in a self-supervised manner. The estimation results in these two scales are ensembled as our final pose estimation. Extensive experiments on widely-used benchmarks demonstrate that our method outperforms state-of-the-art models trained on synthetic data by a large margin and even is on par with several fully-supervised methods.

==> Figures/weakly_sup_seg.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{latex/Images/weakly_sup_seg.pdf}
    \caption{Weakly-supervised Segmentation with 2D Bounding-boxes. We first initialize the segmentation (Seg) network by training on Synthetic data. Then, we iteratively generate pseudo labels for real data and finetune the segmentation network. The outliers in pseudo labels are removed by using bounding-box annotations.}
    \label{fig:weakly_sup_seg}
\end{figure}
